Online Intention Prediction via Control-Informed Learning

This paper presents an online intention prediction framework for estimating the goal state of autonomous systems in real time, even when intention is time-varying, and system dynamics or objectives include unknown parameters. The problem is formulated as an inverse optimal control / inverse reinforcement learning task, with the intention treated as a parameter in the objective. A shifting horizon strategy discounts outdated information, while online control-informed learning enables efficient gradient computation and online parameter updates. Simulations under varying noise levels and hardware experiments on a quadrotor drone demonstrate that the proposed approach achieves accurate, adaptive intention prediction in complex environments.

==> comments.tex <==
Comments to author (Associate Editor)
=====================================

This paper has been reviewed by six reviewers,	who
provided a range of comments regarding the unclear
contribution,  parameter variation analysis, and so on. 
Precisely:
 
1. Lacking theoretical analysis: While convergence
properties are discussed, the theoretical guarantees of the
shifting horizon strategy under frequent goal switching are
not rigorously analyzed. (i dont think we need to respond this)

2. Initialization justification: How is the initial value
$P_0$ for the estimator (8a)–(8d) determined? More
explanation is needed here. (we can add something here, just stating the values we used) (a vector)

3. Unclear contribution:  In the introduction section, the
author emphasizes that while performing online estimation,
there are a few methods that jointly handle the target, the
changing target, and unknown parameters in the dynamics.
However, a brief introduction should be given to what they
have done and what the contribution of this article is
compared to theirs. (we can introduce a little bit about OCIL and PDP)

4. Parameter variation analysis: When considering
time-varying parameters, are there any notable theoretical
or practical differences between the formulation in
Equation (8) and the OCIL framework? It would be helpful to
clarify whether Equation (8) offers specific advantages in
handling such variations compared to the general OCIL
approach. (we dont need to respond to this, our contribution lies in the MPC moving horizon setting)

5. Printing errors: Several grammatical mistakes have been
pointed out throughout the paper by the reviewer. (check for this, you can check the specific review on the submission portal for detail of printing errors)

6. cite all our related papers
